A search for $\mu^+\to e^+\gamma$ with the first dataset of the MEG II experiment

The MEG II experiment, based at the Paul Scherrer Institut in Switzerland, reports the result of a search for the decay $\mu^+\to e^+\gamma$ from data taken in the first physics run in 2021. No excess of events over the expected background is observed, yielding an upper limit on the branching ratio of B($\mu^+\to e^+\gamma$) < $7.5 \times 10^{-13}$ (90% C.L.). The combination of this result and the limit obtained by MEG gives B($\mu^+\to e^+\gamma$) < $3.1 \times 10^{-13}$ (90% C.L.), which is the most stringent limit to date. A ten-fold larger sample of data is being collected during the years 2022-2023, and data-taking will continue in the coming years.

==> author-meg.tex <==
Mu2e+gamma!
\input{institute}

\author[addPSI,addETH]{J.~Adam }
\author[addICEPP]{X.~Bai }
\author[addPisa]{A.~M.~Baldini}
\author[addIrvine,addICEPP]{E.~Baracchini}
\author[addPisa,addPisaUni]{C.~Bemporad}
\author[addPavia,addPaviaUni]{G.~Boca}
\author[addPavia]{P.W. Cattaneo \corref{cor0}} \cortext[cor0]{Corresponding author} \ead{Paolo.Cattaneo@pv.infn.it }
\author[addRoma]{G.~Cavoto }
\author[addPisa,addPisaUni]{F.~Cei} \ead{fabrizio.cei@pi.infn.it}
\author[addPisa]{C.~Cerri}
%\author[addPisa,addPisaUni]{M.~Corbo}
%\author[addPisa,addPisaUni]{N.~Curalli}
\author[addPavia,addPaviaUni]{A.~De Bari}
\author[addGenova, addGenovaUni, addRoma, addPSI]{M.~De Gerone}
%\author[addPisa]{L.~Del~Frate }
\author[addWaseda]{T.~Doke }
\author[addGenova, addGenovaUni]{S.~Dussoni}
\author[addPSI]{J.~Egger }
\author[addGenova, addGenovaUni]{K.~Fratini}
\author[addICEPP]{Y.~Fujii }
%\author[addPisa]{S.~Galeotti }
\author[addPisa,addPisaUni,addPSI]{L.~Galli}
%\author[addPisa,addPisaUni]{L.~Gallucci}
\author[addGenova, addGenovaUni]{F.~Gatti}
\author[addIrvine]{B.~Golden}
\author[addPisa]{M.~Grassi }
\author[addRoma]{A.~Graziosi}
\author[addNovo]{D.N.~Grigoriev }
\author[addKEK]{T.~Haruyama }
\author[addPSI]{M.~Hildebrandt }
\author[addICEPP]{Y.~Hisamatsu }
\author[addNovo]{F.~Ignatov }
\author[addICEPP]{T.~Iwamoto }
\author[addICEPP]{D.~Kaneko }
\author[addICEPP]{K.~Kasami }
\author[addPSI]{P.-R.~Kettle }
\author[addNovo]{B.I.~Khazin }
\author[addNovo]{N.~Khomutov }
\author[addPSI]{O.~Kiselev \fnref{fn4}}
\author[addJINR]{A.~Korenchenko}
\author[addJINR]{N.~Kravchuk}
\author[addIrvine]{G.~Lim}
\author[addKEK]{A.~Maki }
\author[addKEK]{S.~Mihara }
\author[addIrvine]{W.~Molzon}
\author[addICEPP]{T.~Mori }
%\author[addPisa]{F.~Morsani }
\author[addJINR]{D.~Mzavia$^\dagger$}
\author[addPavia,addPaviaUni]{R.~Nard\`o}
\author[addICEPP,addKEK]{H.~Natori }
\author[addPisa,addPisaUni]{D.~Nicol\`o}
\author[addKEK]{H.~Nishiguchi }
\author[addICEPP]{M.~Nishimura}
\author[addICEPP]{Y.~Nishimura \fnref{fn2}}
\author[addICEPP]{W.~Ootani }
%\author[addICEPP]{K.~Ozone }
\author[addLecce,addLecceUni]{M.~Panareo}
\author[addPisa,addPisaUni,addPSI]{A.~Papa }
%\author[addPisa,addPisaUni]{R.~Pazzi $^\dagger$}
\author[addRoma]{G.~Piredda }
\author[addNovo]{A.~Popov }
%\author[addPisa]{F.~Raffaelli}
\author[addRoma,addPSI]{F.~Renga }
\author[addRoma]{E.~Ripiccini }
\author[addPSI]{S.~Ritt }
\author[addPavia]{M.~Rossella}
\author[addPSI]{G.~Rutar}
\author[addICEPP]{R.~Sawada }
%\author[addPSI,addETH]{M.~Schneebeli }
\author[addPisa]{F.~Sergiampietri}
\author[addPisa]{G.~Signorelli}
\author[addWaseda]{S.~Suzuki }
\author[addPisa,addPisaUni]{F.~Tenchini}
\author[addIrvine]{C.~Topchyan}
\author[addICEPP,addPSI]{Y.~Uchiyama }
%\author[addGenova, addGenovaUni]{R.~Valle \fnref{fn3} }
\author[addRoma]{C.~Voena }
\author[addIrvine]{F.~Xiao}
\author[addKEK]{S.~Yamada }
\author[addKEK]{A.~Yamamoto }
\author[addICEPP]{S.~Yamashita }
\author[addIrvine]{Z.~You}
\author[addNovo]{Yu.V.~Yudin }
\author[addRoma]{D.~Zanello }

\address[addPSI] {Paul Scherrer Institut PSI, CH-5232 Villigen, Switzerland}
\address[addETH] {Swiss Federal Institute of Technology ETH, CH-8093 Z\"urich, Switzerland}
\address[addICEPP]{ICEPP, University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan}
\address[addPisa] {INFN Sezione di Pisa, Largo B. Pontecorvo 3, 56127 Pisa, Italy}
\address[addPisaUni] {Pisa, Dipartimento di Fisica dell'Universit\`a, Largo B. Pontecorvo 3, 56127 Pisa, Italy}
\address[addIrvine] {University of California, Irvine, CA 92697, USA}
\address[addPavia] {INFN Sezione di Pavia, Via Bassi 6, 27100 Pavia, Italy}
\address[addPaviaUni] {Pavia, Dipartimento di Fisica dell'Universit\`a, Via Bassi 6, 27100, Pavia, Italy}
\address[addRoma] {INFN Sezione di Roma, Piazzale A. Moro, 00185 Roma, Italy}
\address[addRomaUni] {Roma, Dipartimento di Fisica dell'Universit\`a "Sapienza", Piazzale A. Moro, 00185 Roma, Italy}
\address[addGenova] {INFN Sezione di Genova, Via Dodecaneso 33, 16146 Genova, Italy}
\address[addGenovaUni] {Genova, Dipartimento di Fisica dell'Universit\`a, Via Dodecaneso 33, 16146 Genova, Italy}
\address[addIrvine] {Univeristy of California, Irvine, CA 92697, USA}
\address[addLecce] {INFN Sezione di Lecce, Via per Arnesano, 73100 Lecce, Italy}
\address[addLecceUni] {Lecce, Dipartimento di Fisica dell'Universit\`a, Via per Arnesano, 73100 Lecce, Italy}
\address[addKEK]{KEK, High Energy Accelerator Research Organization 1-1 Oho, Tsukuba, Ibaraki 305-0801, Japan}
\address[addWaseda]{Research Institute for Science and Engineering, Waseda University, 3-4-1 Okubo, Shinjuku-ku, Tokyo 169-8555, Japan}
\address[addNovo] {Budker Institute of Nuclear Physics of Siberian Branch of Russian Academy of Sciences, 630090, Novosibirsk, Russia}
\address[addJINR] {Joint Institute for Nuclear Research, 141980, Dubna, Russia}
\address[addNovSt] {Novosibirsk State Technical University, 630092, Novosibirsk, Russia}

\fntext[fn2]{Present address: Kamioka Observatory, ICRR, University of Tokyo 456 Higashi-Mozumi, Kamioka-cho, Hidacity, Gifu 506-1205, Japan}
\fntext[fn3]{Present address: Lames Holdings S.r.l., 16043 Chiavari, Italy }
\fntext[fn4]{Present address: GSI Helmholtzzentrum für Schwerionenforschung GmbH, D-64291
Darmstadt, BRD }



